A unified theory of the high-dimensional Laplace approximation with application to Bayesian inverse problems

The Laplace approximation (LA) to posteriors is a ubiquitous tool to simplify Bayesian computation, particularly in the high-dimensional settings arising in Bayesian inverse problems. Precisely quantifying the LA accuracy is a challenging problem in the high-dimensional regime. We develop a theory of the LA accuracy to high-dimensional posteriors which both subsumes and unifies a number of results in the literature. The primary advantage of our theory is that we introduce a new degree of flexibility, which can be used to obtain problem-specific upper bounds which are much tighter than previous "rigid" bounds. We demonstrate the theory in a prototypical example of a Bayesian inverse problem, in which this flexibility enables us to improve on prior bounds by an order of magnitude. Our optimized bounds in this setting are dimension-free, and therefore valid in arbitrarily high dimensions.

==> t3-Gauss_new.tex <==
% !TEX root = ../generic.tex

\def\GaussD{\gaussv_{\DPTG}}
\def\EX{\mathcal{E}}
%\def\dlt{f}
\newcommand{\blue}[1]{\textcolor{cyan}{#1}}
\def\dltb{\bar{\dlt}}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
%\def\beqs#1\eeqs{
%    \begin{equation}\begin{split}
%    #1
%    \end{split}\end{equation}
%}
\def\beqsj #1\eeqsj
{
    \begin{equation}
    \setlength{\jot}{10pt}
    \begin{split}
    #1
    \end{split}\end{equation}
}

\def\beqsn#1\eeqsn{
    \begin{equation*}\begin{split}
    #1
    \end{split}\end{equation*}
}

\newcommand{\dltwust}{{\dltwu_3^*}}



\section{Norm Conversions}
\subsection{Definitions and Conventions}
For a symmetric $k$-tensor $\calS$ and a positive definite matrix $A$, we define
\begin{EQA}
\|\calS\|_{A} &=& \sup_{\uv\neq0}\frac{\la \calS, \uv^{\otimes k}\ra}{\|A^{\frac12}\uv\|^k}
\end{EQA}By~\cite{cite}, this definition is equivalent to 
$$\|\calS\|_A =\sup_{\uv_1,\dots,\uv_k\neq0}\frac{\la \calS, \uv_1\otimes \dots\otimes\uv_k\ra}{\|A^{\frac12}\uv_1\|\dots\|A^{\frac12}\uv_k\|}.$$
Note also that for a symmetric matrix $A$, it holds
$$\Tr(A^2)=\la A, A\ra = \|A\|_{\Fr}^2.$$
For a symmetric $p\times p\times p$ tensor $\calS$, a $p\times p$ symmetric matrix $A$, and a vector $\uv$, we let $\la\calS, A\ra$ be the vector with entries
\begin{EQA}\label{tens-mat}\la\calS,A\ra_{i}&=&\sum_{j,k=1}^p\calS_{ijk}A_{jk}\end{EQA} and $\la\calS, \uv\ra$ be the matrix with entries
\begin{EQA}\label{tens-vec}\la\calS,\uv\ra_{ij}&=&\sum_{k=1}^p\calS_{ijk}u_k.\end{EQA} Note that
\begin{EQA}\label{calSuv}\|\la\calS,\uv\ra\|_{A} &=& \sup_{\vv\neq0}\frac{\left\la\la \calS,\uv\ra, \vv\otimes\vv\right\ra}{\|A^{1/2}\vv\|^2}= \sup_{\vv\neq0}\frac{\left\la \calS,\uv\otimes\vv\otimes\vv\right\ra}{\|A^{1/2}\vv\|^2}\leq \|\calS\|_A\|A^{1/2}\uv\|.\end{EQA}
\subsection{A few identities and inequalities}
\begin{lemma}\label{lma:TS}
Let $\calS,\Tens$ be two symmetric $p\times p\times p$ tensors, and $C,A$ be two symmetric positive definite matrices, such that $\la\calS,\uv^{\otimes3}\ra=\la\Tens, (C\uv)^{\otimes3}\ra$ for all $\uv\in\R^p$. Then $\|\calS\|_{CAC}=\|\Tens\|_{A}$.\end{lemma}
\begin{proof}
We have
$$
\|\calS\|_{CAC}=\sup_{\uv\neq0}\frac{\la \calS, \uv^{\otimes3}\ra}{(\uv^{\T}CAC\uv)^{3/2}}=  \sup_{\uv\neq0}\frac{\la \Tens, (C\uv)^{\otimes3}\ra}{((C\uv)^{\T}AC\uv)^{3/2}}= \|\Tens\|_A.
$$\end{proof}
\begin{lemma}\label{lma:AprecB}
Let $A$ and $B$ be two symmetric nonnegative definite matrices. Then $A\preceq \|A\|_BB$. If $A\preceq B$, then $\Tr(A^2)\leq\Tr(B^2)$. 
\end{lemma}
\begin{proof}
We have
$$
\la A, \uv\otimes\uv\ra \leq \|A\|_B\|B^{1/2}\uv\|^2 =\|A\|_B\la B, \uv\otimes\uv\ra = \la \|A\|_BB, \uv\otimes\uv\ra.
$$ Hence $A\preceq\|A\|_BB$. Next, suppose $A\preceq B$. First, note that this implies $\la A, M\ra \leq\la B, M\ra$ for any symmetric $M\succeq0$. Applying this inequality twice gives 
$$\Tr(A^2)=\la A, A\ra \leq \la B, A\ra \leq \la B, B\ra=\Tr(B^2).$$
\end{proof}
\begin{corollary}\label{corr:AprecB}
Let $A, B$ be two symmetric nonnegative definite matrices. Then $\|A\|^2_{\Fr}\leq \|A\|_B^2\|B\|_{\Fr}^2.$
\end{corollary}
\begin{proof}
By Lemma~\ref{lma:AprecB}, we have $A\preceq \|A\|_BB$ and hence 
$$\|A\|^2_{\Fr}=\Tr(A^2)\leq \Tr(( \|A\|_BB)^2) = \|A\|_B^2\Tr(B^2)=\|A\|_B^2\|B\|_{\Fr}^2.$$
\end{proof}
\begin{lemma}\label{lma:SB}
Let $\calS$ be a symmetric $p\times p\times p$ tensor, and $B$ be a symmetric positive definite matrix. Then $\|\calS\|^2_{\Fr}\leq \|\calS\|_B^2\Tr(B)^2\|B\|$.\end{lemma}
\begin{proof}
We have
\begin{EQA}\label{calSFr}
\|\calS\|^2_{\Fr}&=&\sum_{i=1}^p\|\la\calS, \ev_i\ra\|_{\Fr}^2\leq\Tr(B^2)\sum_{i=1}^p\|\la\calS, \ev_i\ra\|_B^2 \\
&\leq &\Tr(B^2)\sum_{i=1}^p\|\calS\|_B^2\|\ev_i\|_B^2=\|\calS\|_B^2\Tr(B^2)\sum_{i=1}^p\ev_i^{\T}B\ev_i = \|\calS\|_B^2\Tr(B^2)\Tr(B).
\end{EQA}
We used Corollary~\ref{corr:AprecB} to get the first inequality and~\eqref{calSuv} to get the second inequality. Next, let $B=\sum_{i=1}^p\lambda_i\uv_i\uv_i^{\T}$ be the eigendecomposition of $B$. Then
$$\Tr(B^2)=\sum_{i=1}^p\lambda_i^2\leq \max_i\lambda_i\sum_{i=1}^p\lambda_i=\|B\|\Tr(B).$$ Applying this inequality in~\eqref{calSFr} concludes the proof.
\end{proof}
\begin{lemma}\label{lma:SI}
Let $\calS$ be a symmetric $p\times p\times p$ tensor, $B$ be a symmetric positive definite matrix, and $I_p$ be the $p\times p$ identity matrix. Then $\|\la \calS, I_p\ra\|^2\leq\|\calS\|_B^2\Tr(B)^2\|B\|$.\end{lemma}
\begin{proof}
We have
\begin{EQA}
\|\la \calS,I_p\ra\|&=&\sup_{\|\uv\|=1}\la\calS, I_p\otimes\uv\ra\leq\sup_{\|\uv\|=1}\sum_{i=1}^p\la\calS, \ev_i\otimes\ev_i\otimes\uv\ra\\
&\leq&\sup_{\|\uv\|=1}\|\calS\|_B\|B^{\frac12}\uv\|\sum_{i=1}^p\|B^{\frac12}\ev_i\|^2\leq\|\calS\|_B\|B^{\frac12}\|\Tr(B).
\end{EQA} Taking the square concludes the proof.
\end{proof}

%\begin{proof}
%We prove the second statement, redefining $\mu=\mu\vert_{\UV}$ and $\nu=\nu\vert_{\UV}$ for brevity. Let $T(x) = \DVL x$. Then $T_{\#}\mu\propto e^{-f_{\DVL}}$ and $T_{\#}\nu\propto e^{-g_{\DVL}}$, where $f_{\DVL}(y)=f(\DVL^{-1}y)$ and $g_{\DVL}(y)=g(\DVL^{-1}y)$. Note that $\nabla^2f_{\DVL}(y)=\DVL^{-1}\nabla^2f(\DVL^{-1}y)\DVL^{-1}\succeq\lambda I$ for all $y\in\DVL\UV$ by assumption. Hence $T_{\#}\mu$ satisfies a log Sobolev inequality (LSI) with constant $1/\lambda$. By Pinsker and the LSI, we have
%\beqs
%\mathrm{TV}(\mu,\nu)^2=\mathrm{TV}(T_{\#}\mu,T_{\#}\nu)^2\leq\frac12\mathrm{KL}(T_{\#}\nu||T_{\#}\mu)\leq\frac{1}{4\lambda}\mathrm{FI}(T_{\#}\nu||T_{\#}\mu),
%\eeqs where
%$$
%\mathrm{FI}(T_{\#}\nu||T_{\#}\mu)=\E_{Y\sim T_{\#}\nu}\left[\left\|\nabla\log\frac{T_{\#}\nu}{T_{\#}\mu}(Y)\right\|^2\right].
%$$ We have $\log(T_{\#}\nu/T_{\#}\mu)(Y)=(f-g)(\DVL^{-1}Y)$ and hence
%$$\nabla\log\frac{T_{\#}\nu}{T_{\#}\mu}(Y)=\DVL^{-1}\nabla(f-g)(\DVL^{-1}Y) \stackrel{d}{=}\DVL^{-1}\nabla(f-g)(X),\qquad X\sim\nu.$$ Therefore
%$$
%\mathrm{FI}(T_{\#}\nu||T_{\#}\mu)=\E_{X\sim \nu}\left[\left\|\DVL^{-1}\nabla(f-g)(X)\right\|^2\right].
%$$
%\end{proof}
\begin{corollary}Let $\mu\propto e^{-f}$. Suppose $\dltwu_{03}\rrdL_0<1$ and $\rrdL_0>6$. Then
\beq\TV(\mu,\gaussG) \leq \frac{\dltwu_{03}(\dimL_0+1)}{3\sqrt{1-\dltwu_{03}\rrdL_0}} +\ex^{-\dimL_0/2 -3(\rrdL_0/3-\sqrt{\dimL_0})^2} + \ex^{-(\rrdL_0-\sqrt{\dimL_0})^2/2}.\eeq
\end{corollary}
\
%\begin{proof}
%First note by Taylor's theorem that $e^{X}-\EX_k(X) = e^y\frac{X^{k}}{k!}$ for some $y$ between $0$ and $X$. Hence $e^{y}\leq 1+e^X$ and $$|e^{X}-\EX_k(X)|\leq \frac{|X|^k}{k!}(1+e^X).$$ Now, consider first the case \( |\xi| \leq 1 \) a.s. By the Cauchy-Schwarz inequality, \eqref{v7jdciuwmedfib5i84k} of Lemma~\ref{PTensG}, and \eqref{6cyvhwyvhejhewycnwsbj}, it holds 
%\beqs
%	\E[|X|^k(1+e^X)]^2& \leq \E [|X|^{2k}] \,\, (2+2\E[e^{2X}])\leq \CONSTi_{k}^{2} \grad^{2k} (2+2\ex^{2 \grad^{2}})\leq 4\CONSTi_{k}^{2} \grad^{2k}\ex^{2 \grad^{2}}.
%\eeqs Thus
%$$\E \bigl[\bigl| \ex^{X} - \EX_{k}(X) \bigr| |\xi|\bigr]\leq \frac{2\CONSTi_k}{k!}\grad^ke^{\grad^2}.$$ For a general \( \xi \), we proceed similarly. Letting \( \rho = k/(k+1) \), we have
%\beqs
%\E[|X|^k(1+e^X)|\xi|]^2 &\leq \E [|X|^{2k} \xi^{2}] \,\, (2+2\E \, e^{2 X})\\
%& \leq \bigl( \E |X|^{2k+2} \bigr)^{\rho} \bigl( \E[ \xi^{2k+2} ]\bigr)^{1 - \rho}(2+2\E [e^{2X} ])\\
%&\leq 4\CONSTi_{k+1}^{2\rho} \grad^{2k}e^{2 \grad^{2}} \, \bigl( \E \xi^{2k+2} \bigr)^{1 - \rho} \, ,
%\eeqs
%and \eqref{7vnf53g6fy363ghfugh62d} follows.
%\end{proof}

%Define \( \nuG = \| \DPTG^{-1} \TG^{2} \DPTG^{-1} \|^{1/2} \) and
%\begin{EQA}
%	\BTG 
%	& \eqdef &
%	\frac{\DPTG^{-1} \TG^{2} \DPTG^{-1}}{\| \DPTG^{-1} \TG^{2} \DPTG^{-1} \|} 
%	=
%	\nuG^{-2} \, \DPTG^{-1} \, \TG^{2} \DPTG^{-1} .
%\label{edsyesuwei8f73mnjcxuyw}
%\end{EQA}

%
%Each \( \TensGt_{i} = \GaussD^{\T} \Tens_{i} \, \GaussD \) can be represented as
%\begin{EQA}
%	\TensGt_{i} 
%	&=& 
%	\GaussD^{\T} \Tens_{i} \, \GaussD
%	=
%	\gaussv^{\T} \TG \, \Tens_{i} \, \TG \gaussv 
%	=
%	\gaussv^{\T} \Tenst_{i} \, \gaussv
%\label{uv6ehryb773fy33ifgiri}
%\end{EQA}
%for \( \Tenst_{i} = \TG \, \Tens_{i} \, \TG \).
%Define
%\begin{EQA}
%	\TensGt
%	& \eqdef &
%	\frac{1}{3} \nabla \Tens(\TG \gaussv)
%	=
%	\TG \, \Tens^{(1)}(\TG \gaussv),
%	\qquad
%	\errSvt = \TensGt - \E \TensGt \, .
%\label{gdyw23bvfuy34hnkh84s}
%\end{EQA}
%Similarly \( \errSvt = \TensGt_{i} - \E \TensGt_{i} \) and Lemma~\ref{LcovTens} implies
%\begin{EQA}
%	\VBHt^{2}
%	\eqdef
%	\Var(\errSvt)
%	&=&
%	\bigl( 2 \langle \Tenst_{i},\Tenst_{\ic} \rangle \bigr)_{i,\ic=1,\ldots,\dimp}
%\label{hyfje3y6thjgky542345}
%\end{EQA}
%with
%\begin{EQA}
%	\langle \Tenst_{i},\Tenst_{\ic} \rangle
%	&=&
%	\tr\bigl( \TG \, \Tens_{i} \, \TG^{2} \Tens_{\ic} \, \TG \bigr),
%	\qquad
%	i,\ic=1,\ldots,\dimp \, .
%\label{gg7ejekbi4jrnktk4rw33}
%\end{EQA}
%For any \( \uv \in \R^{\dimp} \)
%\begin{EQA}
%	\Tenst[\uv]
%	&=&
%	\sum_{i=1}^{\dimp} u_{i} \Tenst_{i}
%	=
%	\TG \, \Tens[\uv] \TG .
%\label{nf7j3mhihijm44ubjrmk}
%\end{EQA}
%Condition \eqref{jkvhey6fgyebetw3egbgh} reads now as
%\begin{EQA}
%	\sup_{\uv \colon \| \VBHG \uv \| \leq 1}
%	\sqrt{2} \, \bigl\| \TG \, \Tens[\uv] \TG \bigr\|
%	& \leq &
%	\tensn 
%	\quad
%	\text{if}\| \VBH \uv \| \leq 1 \, , 
%	\qquad 
%	\| \TG \Tens[\uv] \TG \|_{\Fr} \, ,
%\label{ufj3u8rnioy5i5jg23h}
%\end{EQA}
%while \( \BBH = \QP \VBHt^{2} \QP^{\T} \).
%With this changes, Theorem~\ref{Tdevbount3pm} %and Theorem~\ref{CP2tens} 
%continues to apply.


%For \( \GaussD \sim \ND(0,\TG^{2}) \), define random vector \( \TensG \) by
%\begin{EQA}[rcccl]
%	\TensG 
%	& \eqdef &
%	\frac{1}{3} \nabla \Tens(\GaussD) 
%	=
%	(\TensG_{i})
%	\in \R^{\dimp} \, ,
%	\qquad
%	\TensG_{i}
%	&=&
%	\sum_{j,k=1}^{\dimp} \Tens_{i,j,k} \, \GaussD_{j} \GaussD_{k} \, .
%\label{fkjvjgy4r7r57gtnr53}
%\end{EQA}
%Also the expectation \( \trTv \eqdef \E \, \TensG \) can be written as \( \trTv = (\trT_{i}) \) with
%\begin{EQA}
%	\trT_{i}
%	&=&
%	\sum_{j,k=1}^{\dimp} \Tens_{i,j,k} \, \E \, \GaussD_{j} \GaussD_{k} \, ,
%	\qquad
%	i = 1,\ldots,n.
%\label{fjv7r755hbywgbitee}
%\end{EQA}
%Later we apply another coordinate free representation of \( \trTv \).

%\begin{lemma}
%\label{LTenstrT}
%It holds for any \( \uv \in \R^{\dimp} \) with \( \Tenst^{(2)}(\uv) \eqdef \TG \, \Tens^{(2)}(\uv) \TG \)
%\begin{EQA}
%	\langle \TensG,\uv \rangle
%	&=&
%	\GaussD^{\T} \Tens^{(2)}(\uv) \GaussD 
%	=
%	\gaussv^{\T} \Tenst^{(2)}(\uv) \gaussv,
%	\\
%	\langle \trTv,\uv \rangle
%	&=&
%	\tr (\TG \Tens^{(2)}(\uv) \TG)
%	=
%	\tr \Tenst^{(2)}(\uv) .
%\label{fudvyrf67r7y4hgyerew}
%\end{EQA}
%\end{lemma}
%
%\begin{proof}
%By definition
%\( \TensG = \nabla \Tens(\TG \gaussv) \) for \( \gaussv \) standard normal.
%It follows from \eqref{fkjvjgy4r7r57gtnr53}
%\begin{EQA}
%	\langle \TensG,\uv \rangle
%	&=&
%	\sum_{i,j,k=1}^{\dimp} \Tens_{i,j,k} \, u_{i} \, \GaussD_{j} \GaussD_{k} 
%	=
%	\GaussD^{\T} \Tens^{(2)}(\uv) \GaussD
%	=
%	\gaussv^{\T} \Tenst^{(2)}(\uv) \gaussv
%\label{yfy4erjhhkhji8434ey}
%\end{EQA}
%yielding the assertion.
%\end{proof}


